SpinDOE: A ball spin estimation method for table tennis robot

Spin plays a considerable role in table tennis, making a shot's trajectory harder to read and predict. However, the spin is challenging to measure because of the ball's high velocity and the magnitude of the spin values. Existing methods either require extremely high framerate cameras or are unreliable because they use the ball's logo, which may not always be visible. Because of this, many table tennis-playing robots ignore the spin, which severely limits their capabilities. This paper proposes an easily implementable and reliable spin estimation method. We developed a dotted-ball orientation estimation (DOE) method, that can then be used to estimate the spin. The dots are first localized on the image using a CNN and then identified using geometric hashing. The spin is finally regressed from the estimated orientations. Using our algorithm, the ball's orientation can be estimated with a mean error of 2.4{\deg} and the spin estimation has an relative error lower than 1%. Spins up to 175 rps are measurable with a camera of 350 fps in real time. Using our method, we generated a dataset of table tennis ball trajectories with position and spin, available on our project page.

==> tkiz_fig/geo_hashing.tex <==
\begin{tikzpicture}[tdplot_main_coords, scale = 2.5]
% Create the origin
\coordinate (O) at (0,0,0);


% Create the basis points
\coordinate (B1) at (0.64,0.22,0.77);
\coordinate (B2) at (0.49, 0.85,-0.17);

% Create a feature (F)
\coordinate (F) at ({1/sqrt(3)},{1/sqrt(3)},{1/sqrt(3)});
 
% Draw shaded circle
\shade[ball color = lightgray,
    opacity = 0.5
] (0,0,0) circle (1cm);
 
% Axes in 3 d coordinate system
\draw[-stealth] (0,0,0) -- (1.80,0,0) 
    node[below left] {$x$};
 
\draw[-stealth] (0,0,0) -- (0,1.30,0)
    node[below right] {$y$};
 
\draw[-stealth] (0,0,0) -- (0,0,1.30)
    node[above] {$z$};
 
\draw[dashed, gray] (0,0,0) -- (-1,0,0);
\draw[dashed, gray] (0,0,0) -- (0,-1,0);
 
% Line from the origin to (B1) and (B2)
\draw[thick, -stealth] (0,0,0) -- (B1) node[right] {$B_1$};
\draw[thick, -stealth] (0,0,0) -- (B2) node[right] {$B_2$};
 
% Add small circle at (P)
\draw[fill = lightgray!50] (B1) circle (0.5pt);
\draw[fill = lightgray!50] (B2) circle (0.5pt);
 
\end{tikzpicture}

==> tkiz_fig/orienration_pipeline.tex <==
\begin{tikzpicture}[node distance = 3cm, auto]
        \tikzstyle{block} = [draw, rectangle];
        \tikzstyle{rblock}=[draw, shape=rectangle,rounded corners=0.5em];
\node [rblock] (1) {RGB Image};
\node [block, below=1] (2) {CNN Dot Detector};
\node [rblock, below=2] (3) {Dot Heatmap};
\node [block, below=3] (4) {Blob Detection};
\node [rblock, below=4] (5) {2D Dot Positions};
\node [block, below=5] (6) {Ball surface projection};
\node [rblock, below=6] (7) {3D Dot Position};
\node [block, below=7] (8) {Bayesian Geometric Hashing};
\node [rblock, below=8] (9) {Identified 3D Dot Positon};
\node [block, below=9] (10) {Kabsch's algorithm};
\node [rblock, below=10] (11) {Ball orienation};

\draw [->] (1) -- (2);
\draw [->] (2) -- (3);
\draw [->] (3) -- (4);
\draw [->] (4) -- (5);
\draw [->] (5) -- (6);
\draw [->] (6) -- (7);
\draw [->] (7) -- (8);
\draw [->] (8) -- (9);
\draw [->] (9) -- (10);
\draw [->] (10) -- (11);
\end{tikzpicture}

==> tkiz_fig/setup.tex <==
 \begin{tikzpicture}
  % Incident Beam
  \draw[->, very thick] (-5,0) -- (2,0);
  % Target : Boron + Au
  \shade[top color=gray!60, bottom color=gray!20] (6,1) rectangle (6.25,-1);% Au
  \shade[top color=gray!80, bottom color=gray!40] (6.25,1) rectangle (7.25,-1);% B
  % Scattering Chamber
  %\draw[dotted, red, very thick] (6.6125,0) circle (8cm);
  %\draw[dotted, red, very thick] (6.6125,0) circle (9cm);
  % Telescopes
  \path(6.6125,0)+(170:8)node[right color=black!70, left color=black!20,minimum width=1.2cm,minimum height=.4cm,rotate=80]{$\Delta E$};
  \path(6.6125,0)+(-120:8)node[top color=black!70, bottom color=black!20,minimum width=1.2cm,minimum height=.4cm, rotate=-210]{$\Delta E$};
  \path(6.6125,0)+(170:9)node[right color=black!80, left color=black!40,minimum width=1.2cm,minimum height=1.4cm,rotate=80]{$\mathbf{E}$};
  \path(6.6125,0)+(-120:9)node[top color=black!80, bottom color=black!40,minimum width=1.2cm,minimum height=1.4cm, rotate=-210]{$\mathbf{E}$};
  % Angles
  \draw[dashed, gray, thick] (4,0) -- (6,0);
  \draw[dashed, gray, thick,->] (6,0) -- (170:2);% <-------- This is where it's not working as expected
 \end{tikzpicture}

==> tkiz_fig/view_compensation.tex <==
\begin{tikzpicture}
% Picture's vectors definition
\def\xOne{1}
\def\xTwo{0.5}
\def\yOne{0}
\def\yTwo{-1.3}
\def\zOne{-1}
\def\zTwo{0.5}

% CAMERA COORDINATE SYSTEM
%\draw[thick,->] (0,0) -- (\xOne,\xTwo) node[anchor=north]{$x$};
%\draw[thick,->] (0,0) -- (\yOne,\yTwo) node[anchor=west]{$y$};
%\draw[thick,->] (0,0) -- (\zOne,\zTwo) node[anchor=north,yshift=-2pt,xshift=3pt]{$z$};
\draw[very thick,->] (-\zOne/2,-\zTwo/2) -- (-\zOne/2+\xOne,-\zTwo/2+\xTwo) node[anchor=north west, xshift=-3pt,font=\footnotesize]{$x_c$};
\draw[very thick,->] (-\zOne/2,-\zTwo/2) -- (-\zOne/2+\yOne,-\zTwo/2+\yTwo) node[anchor=west,font=\footnotesize]{$y_c$};
\draw[very thick,->] (-\zOne/2,-\zTwo/2) -- (\zOne/2,\zTwo/2) node[anchor=north,yshift=-2pt,xshift=3pt,font=\footnotesize]{$z_c$};
\draw (-\zOne/2,-\zTwo/2) node[anchor=north west,font=\footnotesize]{$\mathcal{F}_c$};

% CAMERA AXIS ELONGATION
\draw[very thin,solid] (-\zOne/2-2*\xOne,-\zTwo/2-2*\xTwo) -- (-\zOne/2+2*\xOne,-\zTwo/2+2*\xTwo); % x elongation
\draw[very thin,solid] (3*\zOne,3*\zTwo) -- (6*\zOne,6*\zTwo); % optical axis behind projection plane

% REFERENCE LINES
%\draw[thin,dashed] (1.4*\xOne-\zOne/2,1.4*\xTwo-\zTwo/2) -- (6*\zOne+1.4*\xOne,6*\zTwo+1.4*\xTwo); % object x position
\draw[very thin,solid] (6*\zOne-2*\xOne,6*\zTwo-2*\xTwo) -- (6*\zOne+2*\xOne,6*\zTwo+2*\xTwo) node[anchor=west]{}; %object z position

% WORLD OBJECT
\draw[-latex,line width=3pt,blue,line cap=round] (6*\zOne+1.4*\xOne,6*\zTwo+1.4*\xTwo) -- (6*\zOne+1.4*\xOne,6*\zTwo+1.4*\xTwo+1.1) node[anchor=south,font=\footnotesize]{$ P = (X,Y,Z) $};
\node[circle,inner sep=0pt,minimum size=0.2cm,fill=blue] (object) at (6*\zOne+1.4*\xOne,6*\zTwo+1.4*\xTwo+1.1) {};

% PROJECTION LINE BEHIND PROJECTION PLANE
\draw[thick,solid,red] (3*\zOne+0.69*\xOne,3*\zTwo+0.7*\xTwo+0.69) -- (6*\zOne+1.4*\xOne,6*\zTwo+1.4*\xTwo+1.1);

%% PROJECTION PLANE
\filldraw[fill=gray!20,draw=gray!70,opacity=0.8] (3*\zOne-1.5*\xOne-1.5*\yOne,3*\zTwo-1.5*\xTwo-1.5*\yTwo) -- (3*\zOne+1.5*\xOne-1.5*\yOne,3*\zTwo+1.5*\xTwo-1.5*\yTwo) -- (3*\zOne+1.5*\xOne+1.5*\yOne,3*\zTwo+1.5*\xTwo+1.5*\yTwo) -- (3*\zOne-1.5*\xOne+1.5*\yOne,3*\zTwo-1.5*\xTwo+1.5*\yTwo) -- (3*\zOne-1.5*\xOne-1.5*\yOne,3*\zTwo-1.5*\xTwo-1.5*\yTwo);

% PLOJECTION PLANE COORDINATE SYSTEM u,v
\draw[->,thick,green!70!black,dashed] (3*\zOne-1.5*\xOne-1.5*\yOne,3*\zTwo-1.5*\xTwo-1.5*\yTwo) -- (3*\zOne+2*\xOne-1.5*\yOne,3*\zTwo+2*\xTwo-1.5*\yTwo)
     node[anchor=north west, xshift=-3pt,font=\footnotesize]{$u$};
\draw[->,thick,green!70!black,dashed] (3*\zOne-1.5*\xOne-1.5*\yOne,3*\zTwo-1.5*\xTwo-1.5*\yTwo) -- (3*\zOne-1.5*\xOne-1.5*\yOne,3*\zTwo-1.5*\xTwo+2*\yTwo)
     node[anchor=west,font=\footnotesize]{$v$};

% PROJECTION  OBJECT
\draw[-latex,line width=1.5pt,blue,line cap=round] (3*\zOne+0.69*\xOne,3*\zTwo+0.69*\xTwo) -- (3*\zOne+0.69*\xOne,3*\zTwo+0.69*\xTwo+0.69);
\node[circle,inner sep=0pt,minimum size=0.1cm,fill=blue] (object) at (3*\zOne+0.69*\xOne,3*\zTwo+0.7*\xTwo+0.69) {};

% PIXEL OBJECT
\filldraw[red,opacity=0.6] (3*\zOne+6*0.105*\xOne,3*\zTwo+0.75+6*0.105*\xTwo) -- ++(0.105*\xOne,0.105*\xTwo) -- ++(0.105*\yOne,0.105*\yTwo) -- ++(-0.105*\xOne,-0.105*\xTwo) -- ++(-0.105*\yOne,-0.105*\yTwo);

% PROJECTION LINE IN FRONT OF PROJECTION PLANE
\draw[thick,solid,red] (-\zOne/2,-\zTwo/2) -- (3*\zOne+0.69*\xOne,3*\zTwo+0.7*\xTwo+0.69);

% OPTICAL AXIS IN FRONT OF PROJECTION PLANE
\draw[thin,solid] (0,0) -- (3*\zOne,3*\zTwo);

% ANNOTATIONS
% z = f
\draw (3*\zOne-1*\xOne+1.3*\yOne,3*\zTwo-1*\xTwo+1.3*\yTwo) node[gray!70,rotate=28] {$ z = f $};
% (u,v)
\node[green!70!black,anchor=west,font=\scriptsize] at (3*\zOne+0.69*\xOne,3*\zTwo+0.7*\xTwo+0.69) {$ (u,v) $};
% principal point
\draw[very thin] (3*\zOne-0.02*\xOne+0.02*\yOne,3*\zTwo-0.02*\xTwo+0.02*\yTwo) .. controls (3*\zOne-0.1*\xOne+0.3*\yOne,3*\zTwo-0.1*\xTwo+0.3*\yTwo) and (3*\zOne-0.3*\xOne+0.1*\yOne,3*\zTwo-0.3*\xTwo+0.1*\yTwo) ..  (3*\zOne-0.6*\xOne+0.4*\yOne,3*\zTwo-0.6*\xTwo+0.4*\yTwo) 
% optical axis
\draw[very thin] (5.5*\zOne-0.02*\xOne+0.02*\yOne,5.5*\zTwo-0.02*\xOne+0.02*\yOne) .. controls (5.5*\zOne-0.1*\xOne+0.3*\yOne,5.5*\zTwo-0.1*\xTwo+0.3*\yTwo) and (5.5*\zOne-0.3*\xOne+0.1*\yOne,5.5*\zTwo-0.3*\xTwo+0.1*\yTwo) ..  (5.5*\zOne-0.6*\xOne+0.4*\yOne,5.5*\zTwo-0.6*\xTwo+0.4*\yTwo) node[anchor=north,align=center,font=\sffamily\scriptsize] {Optical axis};

\end{tikzpicture}
